UMEM: Unified Memory Extraction and Management Framework for Generalizable Memory

Self-evolving memory serves as the trainable parameters for Large Language Models (LLMs)-based agents, where extraction (distilling insights from experience) and management (updating the memory bank) must be tightly coordinated. Existing methods predominately optimize memory management while treating memory extraction as a static process, resulting in poor generalization, where agents accumulate instance-specific noise rather than robust memories. To address this, we propose Unified Memory Extraction and Management (UMEM), a self-evolving agent framework that jointly optimizes a Large Language Model to simultaneous extract and manage memories. To mitigate overfitting to specific instances, we introduce Semantic Neighborhood Modeling and optimize the model with a neighborhood-level marginal utility reward via GRPO. This approach ensures memory generalizability by evaluating memory utility across clusters of semantically related queries. Extensive experiments across five benchmarks demonstrate that UMEM significantly outperforms highly competitive baselines, achieving up to a 10.67% improvement in multi-turn interactive tasks. Futhermore, UMEM maintains a monotonic growth curve during continuous evolution. Codes and models will be publicly released.

==> tex/sec0_cmo_problem_formulation.tex <==
\section{Problem Formulation}
\label{sec:formulation}
% 
\paragraph{ICL as Token-wise Stochastic Gradient Updates.}
\label{subsec:icl_sgd}

Following \citet{dherin2025learning}, consuming a context sequence
$C=[c_1,\dots,c_n]$ induces an \emph{implicit learning dynamics} on the effective weights.
In particular, Proposition~3.1 in \citet{dherin2025learning} shows that this dynamics is
similar to online gradient descent, \emph{where tokens play the role of data points}:
\begin{equation}
W_{i+1} = W_i - h \nabla_W L_i(W_i),
\qquad
h=\frac{1}{\|A(x)\|^2}.
\label{eq:dherin_sgd}
\end{equation}
Thus, a memory context is not merely conditioning text; it is an implicit optimizer whose update is accumulated token-by-token.%
\footnote{We keep the original notation in \citet{dherin2025learning}, where $L_i$ is a token-dependent surrogate.}

\paragraph{Noisy Data Points Yield High-Variance Implicit Updates.}
\label{subsec:noisy_points}

Existing memory generators are not trained to optimize
downstream reuse; hence the produced context tokens may include task-irrelevant, spurious details~\cite{tang2023large,harutyunyan2024incontextlearningpresencespurious,peters2025generalizationbiaslargelanguage}.
Under Eq.~\eqref{eq:dherin_sgd}, this means the implicit SGD receives \emph{noisy data points}.

Let $g_i \triangleq \nabla_W L_i(W_i)$ be the token-induced update direction at step $i$.
We model spurious tokens as injecting additive noise:
\begin{equation}
g_i \;=\; g_i^\star \;+\; \xi_i,
\qquad
\mathbb{E}[\xi_i]=0,\quad \mathrm{Var}(\xi_i)\ \text{large},
\label{eq:grad_noise}
\end{equation}
where $g_i^\star$ corresponds to the task-invariant schema and $\xi_i$ captures instance-specific variability.
The accumulated implicit update $\Delta W(C) = W_n - W_0 = -h\sum_{i=0}^{n-1} g_i$
then exhibits high variance:
\begin{equation}
\mathrm{Var}\!\left[\Delta W(C)\right]
\;=\;
h^2\,\mathrm{Var}\!\left[\sum_{i=0}^{n-1}\xi_i\right],
\label{eq:update_var}
\end{equation}
which leads to unstable optimization trajectories and poor generalization when the same memory is reused.

\paragraph{Mem-Optimizer: Learning to Denoise the Implicit SGD.}
\label{subsec:mem_objective}

We define a parametric \emph{Mem-Optimizer} $\pi_\phi$ that generates memory tokens
$C \sim \pi_\phi(\cdot \mid T,q)$ from a source trace $T$ of query $q$.
Since memories are stored with key $k=q$ and later reused by cosine retrieval,
the relevant test-time queries are drawn from a \emph{reuse distribution} $q'\sim p_{\mathrm{reuse}}(\cdot\mid q)$,
which captures the set of future queries that are likely to retrieve the same memory under cosine similarity.

Our goal is to synthesize context tokens that yield \emph{low-variance}
implicit updates under reuse:
\begin{equation}
\min_{\phi}\;
\mathbb{E}_{(q,T)}
\mathbb{E}_{C\sim\pi_\phi(\cdot\mid T,q)}
\left[
\mathrm{Var}_{q'\sim p_{\mathrm{reuse}}(\cdot\mid q)}
\big(\Delta W(C; q')\big)
\right],
\label{eq:denoise_objective}
\end{equation}
where $\Delta W(C;q')$ denotes the implicit update induced by context $C$ for query $q'$.
In the next section, we introduce a task-grounded surrogate objective to optimize $\phi$
without accessing $\Delta W$ explicitly.

















% \paragraph{Overview.}
% We formulate the CMO framework as a bi-level optimization problem. We treat in-context inference as an \emph{inner loop} of implicit gradient descent, and the memory extractor as an \emph{outer loop} meta-optimizer.

% % \paragraph{Setup.}
% % Consider a frozen LLM with parameters $\Theta_0$.
% % We define a Memory Bank $\mathcal{B} = \{(k_i, v_i)\}_{i=1}^N$ as a collection of key-value pairs, where:
% % \begin{itemize}
% %     \item The \textbf{Key} $k_i \in \mathcal{Q}$ corresponds to a source query (the problem instance used to generate the memory).
% %     \item The \textbf{Value} $v_i \in \mathcal{M}$ corresponds to the \textbf{memory content} (the optimized token sequence derived from the source).
% % \end{itemize}
% % Given a new query $q'$, the model retrieves relevant memory entries by computing cosine similarity between $q'$ and the stored keys $\{k_i\}$, then performs inference on the prompt formed by concatenating the corresponding values $\{v_i\}$ with $q'$.

% \paragraph{Setup.}
% We consider a frozen LLM with parameters $\Theta_0$ and an external memory bank $\mathcal{B} = \{(k_i, v_i)\}_{i=1}^N$.
% Each memory entry consists of a key $k_i \in \mathcal{Q}$ and a value $v_i \in \mathcal{M}$, where $k_i$ corresponds to the source query that generated the memory, and $v_i$ denotes the associated memory content represented as an optimized token sequence.

% Given a new query $q'$, relevant entries are selected by computing cosine similarity between $q'$ and the stored keys $\{k_i\}$.
% The model then performs inference on the prompt formed by concatenating the retrieved values $\{v_i\}$ with $q'$.


% %-------------------------------------------------------------------------
% \subsection{Inner Loop: ICL as Implicit Weight Update}
% \label{subsec:inner}

% We ground our framework in the \emph{contextual block} abstraction of \citet{dherin2025learning}, modeling a transformer block as $T_W = M_W \circ A$.

% \paragraph{Context as Fast-Weight Update.}
% Providing a memory value $v$ (context) is mathematically equivalent to a rank-1 modification of the frozen weights. Specifically, for a query token $x$, the contextual output is:
% \begin{equation}
% \begin{aligned}
%     T_W(v, x) &= T_{W+\Delta_x W(v)}(x), \\
%     \text{with} \quad \Delta_x W(v) &= \frac{(W \delta A_x(v)) A(x)^\top}{\|A(x)\|^2}.
% \end{aligned}
% \label{eq:rank1_update}
% \end{equation}
% This implies that ICL functions as an \emph{implicit gradient step} with an effective learning rate $\eta \propto \|A(x)\|^{-2}$.

% \paragraph{Inner-Loop Operator.}
% We abstract this inference process as an optimization operator:
% \begin{equation}
%     \Theta_{\mathrm{eff}}(v; q') \;\triangleq\; \mathrm{ImplicitUpdate}(\Theta_0, v; q'),
% \end{equation}
% where the memory value $v$ explicitly dictates the update trajectory applied to $\Theta_0$ for the target query $q'$.

% %-------------------------------------------------------------------------
% \subsection{Retrieval Mechanism}
% \label{subsec:retrieval}

% Given a target query $q'$, we retrieve the top-$K$ memories by matching $q'$ against the keys stored in $\mathcal{B}$. Let $e(\cdot)$ be an $\ell_2$-normalized embedding function. The retrieval operator is defined as:
% \begin{equation}
% \mathcal{R}_K(q') \;\triangleq\; \mathrm{TopK}_{(k_i, v_i)\in\mathcal{B}}\; e(q')^\top e(k_i).
% \label{eq:cos_retrieval}
% \end{equation}
% The effective prompt is the concatenation of the retrieved values: $v_{\mathrm{ret}} = \mathrm{Concat}(\{v_i \mid (k_i, v_i) \in \mathcal{R}_K(q')\})$.

% %-------------------------------------------------------------------------
% \subsection{Outer Loop: Mem-Optimizer}
% \label{subsec:outer}

% We introduce a parametric \emph{extractor} $\pi_\phi$ that acts as a meta-optimizer. For a given interaction trace $T$ of a \textbf{source query} $q$, the extractor synthesizes a memory content $m$:
% \begin{equation}
% m \sim \pi_\phi(\cdot \mid T, q).
% \label{eq:extractor}
% \end{equation}
% This synthesized memory is stored in $\mathcal{B}$ as a new entry where the key is the source query and the value is the generated content: 
% \begin{equation}
% (k, v) \leftarrow (q, m).
% \end{equation}
% Crucially, since $v$ will be retrieved based on its key $k$'s similarity to future queries, $v$ must be effective not just for $k$, but for the entire \emph{semantic neighborhood} of $k$.

% %-------------------------------------------------------------------------
% \subsection{Mem-Optimization Objective}
% \label{subsec:neighborhood}

% \paragraph{Theoretical Basis.}
% \citet{liu2024makes} identify that demonstration utility is governed by the semantic similarity between the test query and the retrieval key. This implies optimal memories must be robust across the local manifold of the source query.

% \paragraph{Empirical Neighborhood.}
% For a source query $q$ (acting as key $k$), we define its empirical neighborhood $\mathcal{N}_K(q)$ as the set of $K$ most similar queries $q'$ from a candidate pool:
% \begin{equation}
% \mathcal{N}_K(q) \;\triangleq\; \mathrm{TopK}_{q' \in \mathcal{Q}}\; e(q)^\top e(q').
% \label{eq:neighbor_def}
% \end{equation}

% \paragraph{Objective \& GRPO Realization.}
% We aim to maximize the expected utility of the generated memory $m$ (value $v$) over the neighborhood of its source $q$ (key $k$). 
% Since $m$ is discrete, we employ \textbf{Group Relative Policy Optimization (GRPO)}.
% For each source $q$, we sample a group of candidate memories $\{m^{(g)}\}_{g=1}^G$ and assign a shared \textbf{neighborhood generalization reward}:
% \begin{equation}
% r(m^{(g)}; q) \;\triangleq\; 
% \underbrace{\frac{1}{K}\sum_{q'\in \mathcal{N}_K(q)}
% \mathcal{U}\!\big(\Theta_{\mathrm{eff}}(m^{(g)};q'), q'\big)}_{\text{Avg. Marginal Gain on Neighborhood}}.
% \label{eq:reward}
% \end{equation}
% The extractor $\pi_\phi$ is updated to maximize $\mathbb{E}[r]$. This explicitly encourages the distillation of invariant schemas that generalize from the source $q$ to its neighbors $q'$.

==> tex/sec1_intro_cmo.tex <==
\section{Introduction}
\label{sec:intro}

Recent advances in large language models (LLMs) have achieved strong performance on static benchmarks.
However, since their parameters remain frozen after training, they cannot learn from new interactions, which restricts their ability to adapt to evolving environments. 
Continual learning (CL) offers a way to overcome this limitation, but parametric approaches such as continual fine-tuning often suffer from catastrophic forgetting~\cite{luo2025empirical}.
Non-parametric memory mechanisms~\cite{zhang2026memrlselfevolvingagentsruntime,xu2025amemagenticmemoryllm} instead externalize experience, enabling continuous adaptation without disrupting existing knowledge.

Existing memory-based approaches predominantly conceptualize memory generation as trajectory compression~\cite{TODO} or semantic summarization~\cite{TODO}, aiming to maximize the fidelity of historical interactions. 
However, we argue that this emphasis on completeness creates a fundamental objective misalignment: preserving raw details often entails preserving irrelevant variability. In the context of In-Context Learning (ICL), such variability creates spurious correlations, biasing the model toward surface-level shortcuts rather than invariant logical structures~\cite{tang2023large,harutyunyan2024incontextlearningpresencespurious}. Consequently, memory functions as a source of distraction rather than guidance, hindering generalization across diverse contexts.

To bridge this gap, we propose \textbf{\textit{Continual Memory Optimization (CMO)}} framework. We redefine memory generation not as indiscriminate trajectory compression, but as active gradient steering.
% meta-optimization. 
Under this framework, we formulate the memory extractor as a \textit{Mem-Optimizer}. Drawing on the view of ICL as implicit gradient descent~\cite{harutyunyan2024incontextlearningpresencespurious}, we conceptualize this component as an runtime-time optimizer. The memory it generates serves effectively as a synthesized gradient update. Consequently, its sole objective is to distill raw interaction history into a precise token sequence that minimizes the variance of implicit updates and steers the frozen LLM toward the underlying task schema, rather than merely summarizing the past.
Concretely, the CMO framework follows a three-stage evolutionary pipeline:
We begin with \textbf{\textit{Semantic Neighborhood Modeling}}, where we retrieve Top-$N$ semantically similar queries from the training set to form validation clusters, establishing a robust evaluation for memory generalization. 
Subsequently, in the \textcolor{red}{\textbf{\textit{Memory Meta-Optimization}}} phase, we freeze the downstream executor and optimize the \textit{Mem-Optimizer} via Group Relative Policy Optimization (GRPO). Specifically, the \textit{Mem-Optimizer} synthesizes candidate memories from the executor's initial trajectories.
These candidates are evaluated using a marginal utility reward, which compares executions with and without the memory across a semantic neighborhood cluster.
In addition, we apply a binary format reward as a hard constraint to ensure structural validity.
Together, the marginal utility reward and the format reward form the final training signal, encouraging the Mem-Optimizer to generate high-utility memories that capture reusable patterns across the neighborhood.
% rather than instance-specific details.
Finally, to enable continuous adaptation, we deploy an \textbf{\textit{Evolutionary Memory Management}} governed by competitive utility ranking. Instead of static storage, the memory bank acts as a dynamic ecosystem where new schemas must outperform existing ones to justify their retention. This ensures that the agent's cognitive capability grows monotonically, as inferior memories are continuously replaced by superior gradients.

\textcolor{red}{We validate the Mem-Optimizer trained via CMO on a comprehensive suite of 7 benchmarks under a CL setting. Empirical results show that our method not only achieves an average gain of \textbf{XX\%} over SOTA baselines but also exhibits a distinct monotonic performance growth curve. This confirms that our framework successfully transforms unstructured interaction history into helpful insight, paving the way for truly self-evolving LLMs.}


% Under this framework, we formulate the \textbf{\textit{memory extractor as a meta-optimizer (Mem-Optimizer)}} that learns to synthesize memories serving as optimal gradient operators. Instead of merely summarizing the past, our objective is to generate context that minimizes the variance of implicit updates and steers the inference model toward the true task schema. 
% While large language models (LLMs) exhibit strong performance under static evaluation, many deployment settings require systems to improve over time as they accumulate interaction experience.
% Continual fine-tuning via parameter updates is a natural solution, but is often impractical in online settings due to deployment cost and catastrophic forgetting~\cite{TODO}.
% This has led to the widespread adoption of non-parametric memory mechanisms~\cite{TODO}, which enable test-time adaptation by externalizing experience without modifying model parameters.
% 具体来说，CMO framework 分为三个stage，首先邻域构建，其次
% Specifically, the extractor synthesizes candidate memories derived from the executor's initial trajectories; these candidates are then rigorously validated via \textbf{\textit{Marginal Utility Verification}} (running with and without memory) on the neighborhood cluster, using the resulting average marginal gain as the reward signal to reinforce high-utility memories.
% Existing memory-based approaches predominantly treat memory generation as trajectory compression~\cite{TODO} or semantic summarization~\cite{TODO}.
% Under this formulation, memories are constructed to preserve as much past information as possible, with limited consideration of their downstream utility.
% As a result, such memories often retain low-utility details and spurious noise, which can interfere with effective generalization at inference time.
% However, we argue that this focus on completeness overlooks a critical issue: preserving raw details often means preserving irrelevant noise. In the context of In-Context Learning, this noise causes the model to overfit to the specific details of past examples. Consequently, the model relies on superficial patterns rather than learning the general reasoning skills needed to solve new, unseen tasks.
% To bridge this gap, we propose \textbf{Continual Memory Optimization (CMO)}. Instead of treating memory as static text, we formulate it as an \textbf{``optimizable gradient operator.''} By modeling the memory extractor as a \textbf{Meta-Optimizer}, we explicitly maximize the gradient utility for future tasks, fundamentally enabling the cognitive evolution of memory.
% In contrast, we argue that the value of memory does not lie in how much information it stores, but in how effectively it abstracts reusable problem-solving structures.
% From this perspective, memory generation should be viewed as a selective distillation process that removes irrelevant variability while preserving task-relevant signals.
% Accordingly, we treat memory as an active component in inference, designed to shape future predictions by providing compact and high-utility contextual guidance.
% Existing memory-based approaches predominantly treat memory generation as trajectory compression~\cite{TODO} or semantic summarization~\cite{TODO}, with the objective of preserving the semantic fidelity of historical interactions.
% In the context of In-Context Learning (ICL), such variability can bias inference-time conditioning toward instance-specific cues.
% Rather than supporting reusable structure, the model is encouraged to rely on surface-level matches instead of reusable logical patterns.
% As a result, memory may function as a source of distraction rather than guidance, limiting its effectiveness when surface details differ across contexts.
% This observation reveals a deeper misalignment in the objective of memory generation.
% Rather than maximizing how much information is retained, we argue that the value of memory lies in how effectively it captures reusable patterns.
% From this perspective, memory generation should be formulated as a selective distillation process, suppressing irrelevant variability while preserving task-relevant signals.
% Accordingly, memory serves as an inference-time mechanism that provides compact, high-utility context to guide future predictions.
